Profinite Techniques for Probabilistic Automata and the Markov Monoid Algorithm

We consider the value 1 problem for probabilistic automata over finite words: it asks whether a given probabilistic automaton accepts words with probability arbitrarily close to 1. This problem is known to be undecidable. However, different algorithms have been proposed to partially solve it; it has been recently shown that the Markov Monoid algorithm, based on algebra, is the most correct algorithm so far. The first contribution of this paper is to give a characterisation of the Markov Monoid algorithm. The second contribution is to develop a profinite theory for probabilistic automata, called the prostochastic theory. This new framework gives a topological account of the value 1 problem, which in this context is cast as an emptiness problem. The above characterisation is reformulated using the prostochastic theory, allowing us to give a simple and modular proof.

==> algorithm.tex <==
The Markov Monoid algorithm was introduced in~\cite{FGO12}.
The presentation that we give here is different yet equivalent.
Consider $\A$ a probabilistic automaton,
the Markov Monoid algorithm consists in computing, through a saturation process, the Markov Monoid of $\A$.

It is a monoid of boolean matrices: 
all numerical values are projected away to boolean values.
Formally, for $M \in \matS{\R}$, define its boolean projection $\boo{M}$,
as the boolean matrix such that $\boo{M}(s,t) = 1$ if $M(s,t) > 0$,
and $\boo{M}(s,t) = 0$ otherwise.
Hence to define the Markov Monoid,
one can consider the underlying non-deterministic automaton $\boo{\A}$
instead of the probabilistic automaton $\A$.

The Markov Monoid of $\boo{\A}$ contains the transition monoid of $\boo{\A}$,
which is the monoid generated by $\set{\boo{\phi(a)} \mid a \in A}$ 
and closed under (boolean matrix) products.
Informally speaking, the transition monoid accounts for 
the boolean action of every finite word.
Formally, for a word $w \in A^*$, the element $\tr{w}$ of 
the transition monoid of $\boo{\A}$
satisfies the following: $\tr{w}(s,t) = 1$ if, and only if there exists
a run from $s$ to $t$ reading $w$ on $\boo{\A}$.

The Markov Monoid generalizes the transition monoid
by introducing a new operator, the stabilization.
On the intuitive level first: let $M \in \matS{R}$, 
it can be interpreted as a Markov chain;
its boolean projection $\boo{M}$ give the structural properties
of this Markov chain.
The stabilization $\boo{M}^\sharp$ accounts for $\lim_n M^n$,
\textit{i.e.} the behaviour of the Markov chain $M$ in the limit.
The formal definition of the stabilization operator relies on basic concepts
from Markov chain theory.

\begin{definition}[Stabilization]
Let $M$ be a boolean matrix.
It is idempotent if $M \cdot M = M$.

Assume $M$ is idempotent,
then we say that $t \in Q$ is $M$-recurrent if
for all $s \in Q$, if $M(s,t) = 1$, then $M(t,s) = 1$.

The stabilization operator is defined only on idempotent elements:
$$M^\sharp(s,t) = 
\begin{cases}
1 & \textrm{if } M(s,t) = 1 \textrm{ and } t \textrm{ is } 
M\textrm{-recurrent,} \\
0 & \textrm{otherwise.}
\end{cases}$$
\end{definition}

The definition of the stabilization
matches the intuition that
in the Markov chain $\lim_n M^n$,
the probability to be in non-recurrent states converges to $0$.
This will be made precise in Subsection~\ref{subsec:characterization}.

\begin{definition}[Markov Monoid]
The Markov Monoid of $\A$ is the smallest set of boolean matrices
containing $\set{\boo{\phi(a)} \mid a \in A}$
and closed under product and stabilization of idempotents.
\end{definition}

We give an equivalent presentation through $\omega$-expressions,
described by the following grammar:
$$E \qquad \longrightarrow \qquad a \quad \mid \quad E \cdot E 
\quad \mid \quad E^\omega\ .$$
We define an interpretation $\tr{\cdot}$ of $\omega$-expressions into boolean matrices:
\begin{itemize}
	\item $\tr{a}$ is $\boo{\phi(a)}$, 
	\item $\tr{E_1 \cdot E_2}$ is $\tr{E_1} \cdot \tr{E_2}$,
	\item $\tr{E^\omega}$ is $\tr{E}^\sharp$, 
	only defined if $\tr{E}$ is idempotent.
\end{itemize}
Then the Markov Monoid is $\set{\tr{E} \mid E \textrm{ an } \omega\textrm{-expression}}$.

The Markov Monoid algorithm computes the Markov Monoid,
and looks for \textit{value $1$ witnesses}:

\begin{definition}[Value 1 Witnesses]
A boolean matrix $M$ is a value $1$ witness if:
for all $s \in I$, $t \in Q$, if $M(s,t) = 1$, then $t \in F$.
\end{definition}

The Markov Monoid algorithm answers ``YES'' 
if there exists a value $1$ witness in the Markov Monoid,
and ``NO'' otherwise.
The following has been proved in~\cite{FGO12}:

\begin{theorem}[\cite{FGO12}]\hfill
\begin{itemize}
	\item If the Markov Monoid algorithm answers ``YES'' on input $\A$, 
	then the probabilistic automaton $\A$ has value $1$,
	\item The converse does not hold in general: 
	there exists a probabilistic automaton
	that has value $1$, such that the Markov Monoid algorithm answers ``NO'',
	\item The Markov Monoid algorithm can be implemented in $\PSPACE$.
\end{itemize}
\end{theorem}

==> characterisation.tex <==


We omit the proof of this proposition, which essentially amounts to gather the results from Section~\ref{sec:prostochastic}.

%\begin{proof}
%We prove the first part of Proposition~\ref{prop:characterisation} by induction on the $\omega$-expression $E$,
%which essentially amounts to gather the results from Section~\ref{sec:prostochastic}.
%
%\medskip
%The base case is $a \in A$, clear.
%
%\textbf{The product case:} let $E = E_1 \cdot E_2$, and $\phi : A \to \matS{\R}$.
%
%We prove that $\boo{\widehat{\phi}(\overline{E})} = \tr{E}$.
%By definition $\overline{E} = \overline{E_1} \cdot \overline{E_2}$,
%so $\widehat{\phi}(\overline{E}) = \widehat{\phi}(\overline{E_1}) \cdot \widehat{\phi}(\overline{E_2})$
%because $\widehat{\phi}$ is a morphism,
%and $\boo{\widehat{\phi}(\overline{E})} = \boo{\widehat{\phi}(\overline{E_1})} \cdot \boo{\widehat{\phi}(\overline{E_2})}$.
%Also by definition, we have $\tr{E} = \tr{E_1} \cdot \tr{E_2}$,
%so the conclusion follows from the induction hypothesis.
% 
%\textbf{The iteration case:} let $E = F^\omega$, and $\phi : A \to \matS{\R}$.
%
%We prove that $\boo{\widehat{\phi}(\overline{E})} = \tr{E}$.
%By definition, $\overline{E} = \overline{F}^\omega$,
%so $\widehat{\phi}(\overline{E}) = \widehat{\phi}(\overline{F}^\omega)$,
%which is equal to $\widehat{\phi}(\overline{F})^\omega$ thanks to Lemma~\ref{lem:limit_fast}.
%Now, $\boo{\widehat{\phi}(\overline{F})^\omega} = \boo{\widehat{\phi}(\overline{F})}^\sharp$ thanks to Theorem~\ref{thm:powers_stochastic_matrix}.
%By induction hypothesis, $\boo{\widehat{\phi}(\overline{F})} = \tr{F}$, which concludes. 
%
%\bigskip
%We prove the second part.
%Consider a sequence $\mathbf{u}$ inducing the polynomial prostochastic word $\overline{E}$.
%Thanks to the first item, $\boo{\widehat{\phi}(\overline{E})} = \tr{E}$,
%implying that $\boo{\lim \phi(\mathbf{u})} = \tr{E}$, which means that $\mathbf{u}$ reifies $\overline{E}$.
%
%\bigskip
%We prove the third part.
%
%Assume that $\tr{E}$ is a value $1$ witness, \textit{i.e.} for all states $t \in Q$, if $\tr{E}(q_0,t) = 1$, then $t \in F$.
%So for $t \notin F$, we have $\lim \phi(\mathbf{u})(q_0,t) = 0$.
%Since we have $\lim \phi(\mathbf{u})(q_0,Q) = 1$, 
%it follows that $\lim \phi(\mathbf{u})(q_0,F) = 1$,
%so $\widehat{\phi}(\overline{E})(q_0,F) = 1$, 
%\textit{i.e.} the polynomial prostochastic word $\overline{E}$ is accepted by $\A$.
%
%Conversely, assume that the polynomial prostochastic word $\overline{E}$ is accepted by $\A$.
%Since it is induced by $\mathbf{u}$, it follows that $\lim \phi(\mathbf{u})(q_0,F) = 1$.
%Consider a state $t \in Q$ such that $\tr{E}(q_0,t) = 1$.
%It follows that $\boo{\lim \phi(\mathbf{u})}(q_0,t) = 1$, so $\lim \phi(\mathbf{u})(q_0,t) > 0$.
%Since $\lim \phi(\mathbf{u})(q_0,F) = 1$, this implies that $t \in F$, hence $\tr{E}$ is a value $1$ witness.
%\hfill\qed\end{proof}

